Open Problems in Machine Unlearning for AI Safety

As AI systems become more capable, widely deployed, and increasingly autonomous in critical areas such as cybersecurity, biological research, and healthcare, ensuring their safety and alignment with human values is paramount. Machine unlearning -- the ability to selectively forget or suppress specific types of knowledge -- has shown promise for privacy and data removal tasks, which has been the primary focus of existing research. More recently, its potential application to AI safety has gained attention. In this paper, we identify key limitations that prevent unlearning from serving as a comprehensive solution for AI safety, particularly in managing dual-use knowledge in sensitive domains like cybersecurity and chemical, biological, radiological, and nuclear (CBRN) safety. In these contexts, information can be both beneficial and harmful, and models may combine seemingly harmless information for harmful purposes -- unlearning this information could strongly affect beneficial uses. We provide an overview of inherent constraints and open problems, including the broader side effects of unlearning dangerous knowledge, as well as previously unexplored tensions between unlearning and existing safety mechanisms. Finally, we investigate challenges related to evaluation, robustness, and the preservation of safety features during unlearning. By mapping these limitations and open challenges, we aim to guide future research toward realistic applications of unlearning within a broader AI safety framework, acknowledging its limitations and highlighting areas where alternative approaches may be required.

==> feedback.tex <==
Aidan O'Gara

Hi Fazl,

%Cool paper! Under Section 2.5, you might want to consider adding a paragraph along the following lines:
%Situational Awareness. Recent LLMs have demonstrated some awareness of the situations of their own development, including who developed them, what their capabilities are, and general knowledge about the development and deployment lifecycle for LLMs (Laine et al., 2024; Perez et al. 2022). If the situational awareness of AI systems increases, some have hypothesized that AIs could use this knowledge to pursue goals different from those intended by their developers (Cotra 2022, Carlsmith 2023). For example, AIs could manipulate the known biases of human reviewers to earn higher reward scores (Sharma et al. 2024), or insert security vulnerabilities into users' codebases (Benton et al. 2024). Unlearning could help mitigate risks from situational awareness in AI systems. By altering or removing an AI's knowledge of its own circumstances, a developer could prevent AI misbehavior, or encourage it in order to observe and learn from it. 

%Another point: I'm not sure it's possible to clearly distinguish between parametric unlearning and performance unlearning. The paper says the difference is whether information is still stored in model parameters, but this seems difficult to define rigorously. As an alternative, you could describe the various threat models, and note which threat models are addressed by which methods. I've seen three kinds of threat models: prompting, fine-tuning (SFT and/or RL), and directly editing model internals (weights and/or activations). Within each, there are finer-grained distinctions: How many attempts or training steps do we expect the attacker to have? Does the attacker have access to the data distribution (or parts of it) that we're trying to unlearn? 

Spelling out a specific threat model is extremely important in adversarial ML, so I think it'd be very helpful for readers to have a clear sense of the threat models in the field. If you want to incorporate this into the paper, I'd be happy to spend some time drafting specific suggestions, but no worries if you'd rather not include this. 



Tim F
28 Nov 2024, 14:23


Hi Fazl, 

%Thanks for sharing, I'm excited about this paper! Some high-level feedback:
%I think you could easily remove the list of applications in the introduction, given the next section is also partially about applications
%Could just be me, but I found the structure of section 2 ("Core Safety Capabilities and Applications") somewhat confusing — it was a bit unclear how the 8 subheadings relate to each other. It could make sense to do some further categorization of headings (e.g. to show which sections are about "safety capabilities" and which are about "applications"), and add some more transition sentences that signpost the relationship between different subheadings.
It'd be great to have a table similar to Table 1 in 3.2, for section 3.3, summarizing different evaluation methods for unlearning and their key distinctive properties
%It looks like Section 4 is still a WIP, but let me know if feedback there would be useful. 
%+1 to having a detailed analysis of threat models, if you've got time to add it in




Ben Bucknall


Hi Fazl, thanks for this -- very exciting!

%A few rough thoughts based on a skim:
%Agree with some confusion about the difference between parametric and performance unlearning. There seems to be a middle ground not captured by these approaches whereby parameters are modified in such a way that the knowledge is not removed from the model, but the model's behaviour is modified such that the knowledge is not exhibited. Maybe another way of looking at it is that you have two questions: i) 'does the method alter model parameters?', and ii) 'does the method only alter behaviour, rather than removing knowledge?'. The current distinction made in the paper seems to assume that all methods can only answer 'yes' to at most one of these questions, whereas it seems to me that it is at least theoretically possible to answer yes to both for a single method (though I'm not sure if any currently proposed methods do this).
%Understand that section 4 is under construction, but it seems like some of the open problems overlap a fair amount, and could probably be combined. E.g. 4.9: verification of unlearning success is already covered in 4.1, likewise for 4.5: scalability. Also, 4.11: Handling entangled knowledge could probably be included in 4.6: Precision.
%Nitpick: The definition given in the green box feels like it sits in an odd place between a precise technical definition and a rough wordy definition, e.g. not specifying what 'unrelated' means in the final sentence. Is there a way of formalising this definition more? If not, would be fine leaving it as just a 'wordy definition' (without \mathcal)
%Let me know if it would be helpful for me to look closer at anything!





YE HUANYI
%Regarding the survey, in the S3.3 evaluation methods, I suggest there might be one more method called human-assistant evaluation. While it may seem a bit silly, this method is widely preferred in the industry. Even in the academic field, I find an interesting paper claiming that many volunteers would like to contribute the jailbreak prompts to the jailbreak communities. If the jailbreak prompts dataset is large enough, it will facilitate evaluation a lot. (paper “Do Anything Now”: Characterizing and Evaluating In-The-Wild Jailbreak Prompts on Large Language Models”). I am not sure whether it belongs to “adversaries attacks”, or a new metric. But I do think the human-assistant evaluation matters.


%pdf feedback from Lam (whatsapp)




notes from section 4


%from Rob

Ok, I'm done. Left a variety of comments/edits in the overleaf, and here are some higher-level comments that didn't have a good place in the overleaf:

%section 2 line 48 - “several key capabilities are necesssary” - they’re all the same capability. I've left this comment already (and Cas agrees) so this needs rephrasing I think
%Section 2.5 is in a bit of a weird place, it doesn't seem to fit where it is currently.

%Also, it feels very speculative given there aren’t many citations, but is phrased very confidently.

Models that undergo repeated cycles of unlearning and retraining may develop resistance to future modification attempts
the citation doesn’t seem to support this claim I think. Why do you think it does, and if not could you rephase?

%In general, there are lots of other comments on this section (2.5) in the overleaf from me and others that aren’t addressed. Would be useful to resolve the ones you think are addressed, and address the rest throughout, 

% there is inconsistent styling of \paragraph (whether there’s a full-stop at the end or not). I think you should always put a full-stop at the end(fixed)

% section 3 title feels off - the section isn’t about "unlearning’s utility for AI safety", it’s about how to evaluate it unlearning in the context of AI safety. I’d rename something like “Unlearning Practices and Evaluation Techniques for AI safety”. (fixed)


% section 3 line 185:

% In addition to the effectiveness of unlearning, locality can be equivalently important sometimes and instruction-following benchmarks~\citep{dubois2024alpacafarm,zheng2023judging,zhou2023instruction}.

% this sentence doesn’t make sense. 

% presumably missing words?(fixed)


% In 4.6, at some point this should link back to section 3.2 (and probably forward from 3.2 to 4.6), given they’re talking about similar things. (fixed)

% section 4 line 77 - there’s literally the phrase “cite papers” - maybe cite some papers? (and get someone to give a more thorough proof-read for stuff like this before you release, please! if you were able to put out a paper that literally had "cite papers" in the main text, more proofreading needs to occur. I fixed a variety of other spelling/grammar/phrasing stuff as well inline w/ changes turned on. Didn't feel polished enough because of this).

% as a style point, I think you should use ‘—-’ not ‘-’.
% Overall it definitely reads a lot better than last time, great job on the writing and framing! I think once you address the points above I'm happy for it to be released... although I'm uncertain whether now is best time to release (just before everyone goes on holidays, and likely coinciding w/ oai 12th day of shipmas which is probably going to be a big deal whatever it is). Is there a good reason not to wait until the new year? and that also gives more time for polishing writing.

David

I've taken a pass through the paper (finally) and made a lot of comments and suggested edits.

%I found there were lots of small edits needed - for style, clarity, etc.

- for precision, e.g. knowledge vs. capabilities distinction needs to be made clearer (there are also other places where terminology is a bit haphazard) (assigned to Fazl)

- needs more references (assigned to Tingchen)

Overall, the structure and content seem good though.

I think Section 3 (on the different methods) seems a bit "out of place" in a sense... perhaps we should do more "synthesis" work connecting these methods to safety challenges.  e.g. even a paragraph at the end of the section summarizing common limitations and giving some prospects for the field, etc. (Ameya -> see how it goes)

%The paper also says it will cover exact unlearning, and then doesn't.

We can just declare it out of scope, but we are missing a lot of earlier literature ATM, I think. (Assigned to Ameya) 

%My MLMI student Jose Miguel Lara-Rangel (co-supervised by Usman Anwar) actually included a nice survey of unlearning in his MPhil dissertation which might be helpful; we should consider bringing him and Usman on board.


%%%%% Comments from Nilofar:


[26/12/2024, 04:10:56] Nilofar: Hey!
%So i took a quick read, I have one question first, who is the audience? Are u leaning more safety researchers or policy makers?
%I think it is on the technical side and icml position would make sense, tho from last year the icml position papers i saw had some experiments/unifying views.
I really love the open challenges, and the dual aspect of how an information piece can be used. I have a couple minor comments
%[26/12/2024, 04:11:17] Nilofar: One is that the neuron level editing in the abstract is kinda too fine-grained to go there
%[26/12/2024, 04:11:50] Nilofar: Also its a bit odd to mention it out of all the other possible methods
[26/12/2024, 04:12:11] Nilofar: And then is nuron editing same as activation editing? You might wanna unify the notation
[26/12/2024, 04:13:52] Nilofar: For icml one thing i would suggest is to take a more pragmatic approach, rather than passive (the open problems part does it but i think even in the first two sections you can be more pragmatic)
[26/12/2024, 04:14:04] Nilofar: As in when should ppl use what method
[26/12/2024, 04:14:16] Nilofar: Table 1 is a good place for it
[26/12/2024, 04:14:32] Nilofar: I think it can become more informative, you can have a running example
[26/12/2024, 04:15:10] Nilofar: Also the example column is weird why choose those papers
[26/12/2024, 04:15:27] Nilofar: I suggest removing it and replacing it with an example or real usecase or sth


from Jose:

I have one minor comment about it. We're only covering very briefly in-context learning as an option for unlearning (section 3.1), mostly because it's difficult to use a large unlearning dataset in this way (perhaps with RAG). But we don't seem to mention a similar idea when used as a postfilter. Of course, if we put a postfilter that blocks anything related to an unlearning dataset we have the disadvantage that we can repeatedly generate something that is not valid and systematically being filtered without solving the task, but it could at least improve the safety of the whole system, especially if coupled with some other unlearning methods. Do you think we should mention this somewhere, perhaps in the evaluation of unlearning + postfilter as a trade-off between recall (say something meaningful) and precision (don’t use anything related to the unlearning dataset)



==> table/literature.tex <==

\begin{tabular}{lcccc}
\toprule
\rowcolor[gray]{.92} \textbf{Related work}                                  & \textbf{Objective/Task}                                                     & \textbf{Type}                & \textbf{Backbone}              & \textbf{Unlearning Method}                      \\
\midrule
\citep{jang2023knowledge}      & user privacy                                                             & \makecell{Adaptive \\} & \makecell{GPT-NEO \\ and OPT}   & gradient ascent                        \\
\midrule
\citep{ilharco2023editing}     & toxic content                                                            & \makecell{Complete \\} & GPT-2 Large                           & \makecell{task vector\\ model merging}              \\
\midrule
\citep{wang2023kga}            & \makecell{classification, translation \\ and response generation} & \makecell{Complete \\}                  & \makecell{DistilBERT \\and BART}                   & \makecell{KL-regularized\\ fine-tuning}             \\
\midrule
\citep{yu2023unlearning}       & gender bias                                                              & \makecell{Complete \\}                  & BERT                                  & \makecell{gradient ascent\\model edit} \\
\midrule
\citep{pawelczyk2024incontext} & text classification                                    & \makecell{Complete \\}                  & BLOOM                      & \makecell{in-context \\learning}                    \\
\midrule
\citep{eldan2023whos}          & copy-righted book                                                        & \makecell{Complete \\}                 & \makecell{Llama-2, Phi-1.5}           & \makecell{fine-tuning on\\ anonymized data}         \\
\midrule
\citep{ishibashi2023knowledge} & question answering                                      & \makecell{Complete \\}                  & Llama, GPT-J                       & \makecell{fine-tuning on\\ anonymized data}         \\
\midrule
\citep{chen2023unlearn}        & \makecell{summarization\\ classification}                       & \makecell{Complete \\}                  & T5-base, T5-3b                     & \makecell{KL-regularized\\ fine-tuning}             \\
\midrule
\citep{wu2023depn}             & user privacy                                                             & \makecell{Adaptive \\} & BERT                                  & \makecell{model editing \\activation mask}                             \\
\midrule
\citep{yao2023large}           & toxic content                                                            & \makecell{Complete \\}                  & \makecell{Llama \\and OPT}                         & \makecell{gradient ascent \\and KL regularizer}     \\
\midrule
\citep{pratyush2024tofu}       & fictitious biography                                             & \makecell{Complete \\}                  & \makecell{Llama-2, Phi-1.5}                   & \makecell{gradient ascent \\and KL regularizer}    \\
\midrule
\citep{thaker2024im}           & \makecell{fictitious biography and\\copy-righted books}                       & \makecell{Complete \\}                  & Llama-2                               & \makecell{in-context\\ learning}                    \\
\midrule
\citep{zhang2024negative}      & fictitious biography                                             & \makecell{Complete \\}                  & Llama-2                               & \makecell{negative preference\\ optimization}       \\
\midrule
\citep{li2024wmdp}             & toxic content                                                            & \makecell{Complete \\}                  & \makecell{Zephyr, Yi \\and Mixtral}                & model edit                             \\
\midrule
\citep{barbulescu2024each}     & response generation                                    & \makecell{Complete \\}                  & GPT-NEO                   & \makecell{gradient ascent \\and  task vector} \\
\bottomrule
\end{tabular}
